Coded Computing Meets Quantum Circuit Simulation: Coded Parallel Tensor Network Contraction Algorithm

Parallel tensor network contraction algorithms have emerged as the pivotal benchmarks for assessing the classical limits of computation, exemplified by Google's demonstration of quantum supremacy through random circuit sampling. However, the massive parallelization of the algorithm makes it vulnerable to computer node failures. In this work, we apply coded computing to a practical parallel tensor network contraction algorithm. To the best of our knowledge, this is the first attempt to code tensor network contractions. Inspired by matrix multiplication codes, we provide two coding schemes: 2-node code for practicality in quantum simulation and hyperedge code for generality. Our 2-node code successfully achieves significant gain for $f$-resilient number compared to naive replication, proportional to both the number of node failures and the dimension product of sliced indices. Our hyperedge code can cover tensor networks out of the scope of quantum, with degraded gain in the exchange of its generality.

==> 2-node.tex <==
Parallel tensor network contraction algorithm\cite{chenzhang} is mostly used for quantum  simulation in current studies\cite{stepdependent,jet,adaptive,indexslicing}. Tensor networks of the quantum domain that are computationally expensive enough to require Chen and Zhang's algorithm\cite{chenzhang}  are mainly of Projected Entangled-Pair States (PEPS) structure\cite{mpspeps}, which can represent quantum systems of great contemporary interests such as 2-dimensional qubit arrays. PEPS structure consists of only 2-node closed indices. For this special class of tensor networks we provide an upperbound of $f$-resilient number via Theorem 1, based on the efficient coding scheme we call \emph{2-node code}.


\begin{theorem}
    For the special case of the problem stated in \ref{sec:system}, where $m_{i}=2$ for all $i$, the achievable $f$-resilient number is bounded above by
\begin{equation}\label{eq:threshold2}
f+2\prod_{i=1}^{n}L_{i}-1.
\end{equation}

The corresponding gain compared to naive replication is
\begin{equation}\label{eq:gain2}
\Delta=(\prod_{i=1}^{n}L_{i}-1)(f-1).
\end{equation}
\end{theorem}

We demonstrate an example for Theorem~2 with a tensor network similar to the one used in previous subsection, but with $(m_1=2, L_1 =4)$ and $(m_2=2, L_2=3)$. Equation for sliced tensor networks is now as below:
$$
\boldsymbol{\sigma}_{a,b}=\sum_{-}(\boldsymbol{A}^{(1)}_{a,-}\boldsymbol{A}^{(2)}_{a,-}\boldsymbol{B}^{(1)}_{b,-}\boldsymbol{B}^{(2)}_{b,-})\boldsymbol{T}_{-},
$$
where $a\in\{1,2,3,4\}$ $b\in\{1,2,3\}$.

Our encoded tensor networks replace the sliced tensors as follows using an arbitrary constant $x$:
$$
\Tilde{\boldsymbol{A}}^{(1)}_{-}=\boldsymbol{A}^{(1)}_{1,-} + \boldsymbol{A}^{(1)}_{2,-}x + \boldsymbol{A}^{(1)}_{3,-}x^{2}+\boldsymbol{A}^{(1)}_{4,-}x^{3}
$$
$$
\Tilde{\boldsymbol{A}}^{(2)}_{-}=\boldsymbol{A}^{(2)}_{1,-}x^3 + \boldsymbol{A}^{(2)}_{2,-}x^2 + \boldsymbol{A}^{(2)}_{3,-}x+\boldsymbol{A}^{(2)}_{4,-}
$$
$$
\Tilde{\boldsymbol{B}}^{(1)}_{-}=\boldsymbol{B}^{(1)}_{1,-} + \boldsymbol{B}^{(1)}_{2,-}x^4 + \boldsymbol{B}^{(1)}_{3,-}(x^4)^2
$$
$$
\Tilde{\boldsymbol{B}}^{(2)}_{-}=\boldsymbol{B}^{(2)}_{1,-}(x^4)^2 + \boldsymbol{B}^{(2)}_{2,-}x^4 + \boldsymbol{B}^{(2)}_{3,-}.
$$

Equation of the encoded tensor network will be as follows:
$$
\Tilde{\boldsymbol{\sigma}}=\sum_{-}(\Tilde{\boldsymbol{A}}^{(1)}_{-}\Tilde{\boldsymbol{A}}^{(2)}_{-}\Tilde{\boldsymbol{B}}^{(1)}_{-}\Tilde{\boldsymbol{B}}^{(2)}_{-})\boldsymbol{T}_{-}
$$$$
=(\boldsymbol{\sigma}_{1,1}+\boldsymbol{\sigma}_{2,1}+\boldsymbol{\sigma}_{3,1}+...+\boldsymbol{\sigma}_{4,3})x^{11}+(\text{other order terms})
$$
$$
=\boldsymbol{\sigma}_{\text{final}}x^{11}+(\text{other order terms})=\text{poly}(x^{22})
$$

Hence, with any $(22+1)$ successful workers each of different constant $x$, $\boldsymbol{\sigma}_{\text{final}}$ can be retrieved at the master. $f$-resilient number in this case is $(f+22+1)$ workers for $f$  failures, and the gain compared to naive replication is:
$$
\Delta=12(f+1)-(22+f+1)=11(f-1) \hspace{4pt}(\text{workers}).
$$
The result is consistent with Theorem 2 as shown below:
$$
\Delta=(12-1)(f-1)=11(f-1)
$$

In addition, PEPS structure tensor networks used in practice are usually consist of uniform dimension for all closed edges\cite{}. Hence, we provide a corollary from Theorem 1 for practitioners of the field.

\begin{corollary}
(For Quantum Simulation) As a corollary from Theorem 1, for the case where $m_i=2, L_{i}=L > 2$ for all $i$, the achievable $f$-resilient number is bounded above by
\begin{equation}
f+2L^{n}-1. 
\end{equation}

The corresponding gain compared to naive replication is
\begin{equation}
\Delta=(L^n-1)(f-1).  
\end{equation}
\end{corollary}


==> backup.tex <==
Our coding strategies differ by whether the sliced indices are all two-node indices or not. If sliced indices are all two-node indices, we found out that all the desired terms can be confined into one coefficient of the resulting polynomial. The gain in $f$-resilient number compared to naive replication is significant as a result, exponential by the number of sliced indices. However, as we have assumed earlier, sliced indices are likely to be multiple-node indices for an arbitrary tensor network. Although coding scheme for multiple-node indices might be more valuable, we have yet failed to find a coding scheme where we can confine all desired terms into one coefficient of the resulting polynomial for such cases. Instead, coding scheme we found confines each of the desired terms into each individual coefficients respectively, hence the resulting polynomial is significantly higher compared to two-node indices case. If the number of node failures is big enough, our method still provides big gain of $f$-resilient number compared to naive replication. However, the $f$-resilient number increases by the product of the number of tensors connected to each sliced indices, hence our method may not be effective for indices connecting large number of tensors. In that case, we propose an alternative coding scheme, which the $f$-resilient number does not exponentially increase by the number of the tensors connected to sliced indices, but which it does get affected more by number of node failures. Thus, whether which scheme is more efficient depends both on the distributed system in use and the tensor network structure.

Tensor network formalism is not only for quantum simulation application, and any indices can have arbitrary dimension, hundreds and millions if wanted.  Although references note that the parallelization scheme is not only for quantum simulation but also can be applied to arbitrary tensor networks, by far practical implementations of it on large scale distributed clusters are mostly in the field of quantum circuit simulation, if not all of them. As coded computation is a technology for distributed computation large enough to suffer from computational node failures, our coding schemes are explicitly for tensor networks for quantum circuit simulation, which all indices are two dimensional in most of the cases. Expanding codes for tensor networks with indices of higher dimension is left for future works.

Assumption 2 is from the property of tensor network contraction that its computational complexity is decided by the largest number of indices of the intermediate tensors produced during the process\cite{adaptive}. Hence, it is only reasonable to assume that indices connecting largest number of tensors are likely to make cheapest sliced tensor networks if sliced. However, selecting optimal set of indices to slice to produce the cheapest sliced tensor network for an arbitrary tensor network is another NP-complete problem\cite{parallelnphard}. According to several works on the heuristics of selecting indices to slice as close to optimal as possible\cite{}, for some cases, indices connecting fewer tensors than others might be evaluated to produce cheaper sliced tensor networks when sliced. Hence, we provide coding schemes not only for multiple-node indices, but also for two-node indices as well. It is notable that for certain applications of tensor network, especially quantum many-body simulation and machine learning\cite{mlexample2,mlexample3,mlexample4}, tensor network structures consisted of only two-node indices such as Matrix Product States (MPS) and Projected Entangled Pair States (PEPS) are widely used\cite{}. However, application of tensor network formalism which parallelization scheme is mostly implemented, if not all, is quantum circuit simulation, where tensor networks often require multiple-node indices. Some of the tensor networks for quantum circuit simulation can be simplified to have only two-node indices by using controlled-Z gates and exploiting diagonal quantum gates\cite{diagonal}. Even so, most complicated tensor networks that requires large scale distributed system may consist of multiple-node indices, and by our assumption 2, we expect coding scheme for such indices to be valuable.




==> hyperedge.tex <==
As tensor network framework is also being recognized by diverse communities outside of quantum, tensor network structure with one or more hyperedges might gain interest in the future. Also, for the completeness of our work, we recognize a need for more general coding scheme than the 2-node code.  

Hence, we provide much general coding scheme, \emph{hyperedge code} as we call it, that applies to an arbitrary tensor network. The only restriction 
in the generality is to not slice adjacent indices. Upperbound of $f$-resilient number for an arbitrary tensor network is provided via Theorem 2 based on the hyperedge code.

\begin{theorem}
    For the problem stated in \ref{sec:system}, the achievable $f$-resilient number is bounded above by
\begin{equation}\label{eq:threshold1}
f+\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)}.
\end{equation}

The corresponding gain compared to naive replication is
\begin{equation}\label{eq:gain1}
\Delta=(\prod_{i=1}^{n}L_{i}-1)(f+1)-\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)}+1.
\end{equation}
\end{theorem}

Note that the coding gain is larger when there is
a higher number of failures. Moreover, the topology of sliced tensor networks remains unchanged when encoded with our scheme. This is because the encoding process involves replacing original sliced tensors with encoded tensors of identical dimensions. Hence, our codes preserves the computation cost of individual workers. 

We demonstrate an example code construction that achieves the $f$-resilient number given in Theorem 1 for $n=2$. 
Let us denote two indices we slice as $a$ and $b$, each of which with prameters $(m_1=3,L_1=2)$ and $(m_2=4,L_2=2)$ respectively. Then, tensors sliced by these indices can be referred as $\boldsymbol{A}^{(i)}_{a,-} (i=1,2,3)$ and $\boldsymbol{B}^{(j)}_{b,-} (j=1,2,3,4)$ respectively. There are $N=L_a\cdot L_b=4$ sliced tensor networks which can be written as below:
$$
\boldsymbol{\sigma}_{a,b}=\sum_{-}(\boldsymbol{A}^{(1)}_{a,-}\boldsymbol{A}^{(2)}_{a,-}\boldsymbol{A}^{(3)}_{a,-}\boldsymbol{B}^{(1)}_{b,-}\boldsymbol{B}^{(2)}_{b,-}\boldsymbol{B}^{(3)}_{b,-}\boldsymbol{B}^{(4)}_{b,-})\boldsymbol{T}_{-},
$$
where $a\in\{1,2\}$ $b\in\{1,2\}$, hence
$$
\boldsymbol{\sigma}_{\text{final}}=\boldsymbol{\sigma}_{1,1}+\boldsymbol{\sigma}_{2,1}+\boldsymbol{\sigma}_{1,2}+\boldsymbol{\sigma}_{2,2}.
$$

Our encoded tensor networks replace the sliced tensors by encoded tensors as follows using an arbitrary constant $x$:
$$
\Tilde{\boldsymbol{A}}^{(i)}_{-}=\boldsymbol{A}^{(i)}_{1,-} + \boldsymbol{A}^{(i)}_{2,-}x
$$
$$
\Tilde{\boldsymbol{B}}^{(j)}_{-}=\boldsymbol{B}^{(k)}_{1,-} + \boldsymbol{B}^{(j)}_{2,-}x^{1+3}
$$
where $i=1,2,3$ and $j=1,2,3,4$.

The equation of the encoded tensor network will be as follows:
$$
\Tilde{\boldsymbol{\sigma}}=\sum_{-}(\Tilde{\boldsymbol{A}}^{(1)}_{-}\Tilde{\boldsymbol{A}}^{(2)}_{-}\Tilde{\boldsymbol{A}}^{(3)}_{-}\Tilde{\boldsymbol{B}}^{(1)}_{-}\Tilde{\boldsymbol{B}}^{(2)}_{-}\Tilde{\boldsymbol{B}}^{(3)}_{-}\Tilde{\boldsymbol{B}}^{(4)}_{-})\boldsymbol{T}_{-}
$$
$$
=\boldsymbol{\sigma}_{1,1}+\boldsymbol{\sigma}_{2,1}x^3+\boldsymbol{\sigma}_{1,2}x^{4}+\boldsymbol{\sigma}_{2,2}x^{19}+(\text{other order terms})$$
$$
= \text{poly}(x^{19})
$$
Hence, with any $(19+1)$ successful workers, all the 4 desired results of sliced tensor networks, $(\boldsymbol{\sigma}_{1,1},\boldsymbol{\sigma}_{2,1},\boldsymbol{\sigma}_{1,2},\boldsymbol{\sigma}_{2,2}$), can be retrieved and then summed up at the master to acquire $\boldsymbol{\sigma}_{\text{final}}$. $f$-resilient number in this case is $(f+19+1)$ workers for $f$ node failures, and the gain compared to naive replication is:
$$
\Delta=4(f+1)-(f+20)=3f-16 \hspace{4pt}(\text{workers}).
$$
The result is consistent with Theorem 1 as shown below:
$$
\Delta=(4-1)(f+1)-\frac{(3^2-1)}{(3-1)}\frac{(4^2-1)}{(4-1)}+1=3f-16.
$$

==> practical.tex <==
\subsection{Partial Coding}

As shown above, 2-node code is more efficient than hyperedge code. In practice, there may be a case where both 2-node indices and hyperedges are sliced. In such case, coding only 2-node indices with 2-node code and leaving the hyperedges uncoded might provide lower $f$-resilient number than coding all sliced indices by hyperedge code. Hence we provide a corollary from Theorem 1 and Theorem 2, \emph{partial coding}, as we call it.

\begin{corollary}
(Partial Coding $k$ 2-node Indices) For the problem stated in \ref{sec:system}, if $m_i=2 (i=1,2,..,k)$ and $m_i>2(i=k+1,..,n$), the achievable $f$-resilient number is bounded above by
\begin{equation}
\min\bigg(f+\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)},\hspace{5pt}(\prod_{j=k+1}^{n}L_j)(f+2\prod_{l=1}^{k}L_{l}-1)\bigg).
\end{equation}
\end{corollary}

First term in $\min$ is the $f$-resilient number upperbound by hyperedge code from Theorem 1. Second term is the $f$-resilient number upperbound when only 2-node sliced indices $(i=1,2,..,k)$ are coded by 2-node code, leaving the remaining $(n-k)$ sliced hyperedges uncoded. Hence, the second term represents $(\prod_{j=k+1}^{n}L_j)$ sets of sliced tensor networks, each coded by 2-node code on its $k$ sliced 2-node indices.


\subsection{Partial Coding}

As shown above, 2-node code is more efficient than hyperedge code. In practice, there may be a case where both 2-node indices and hyperedges are sliced. In such case, coding only 2-node indices with 2-node code and leaving the hyperedges uncoded might provide lower $f$-resilient number than coding all sliced indices by hyperedge code. Hence we provide a corollary from Theorem 1 and Theorem 2, \emph{partial coding}, as we call it.

\begin{corollary}
(Partial Coding $k$ 2-node Indices) For the problem stated in \ref{sec:system}, if $m_i=2 (i=1,2,..,k)$ and $m_i>2(i=k+1,..,n$), the achievable $f$-resilient number is bounded above by
\begin{equation}
\min\bigg(f+\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)},\hspace{5pt}(\prod_{j=k+1}^{n}L_j)(f+2\prod_{l=1}^{k}L_{l}-1)\bigg).
\end{equation}
\end{corollary}

First term in $\min$ is the $f$-resilient number upperbound by hyperedge code from Theorem 1. Second term is the $f$-resilient number upperbound when only 2-node sliced indices $(i=1,2,..,k)$ are coded by 2-node code, leaving the remaining $(n-k)$ sliced hyperedges uncoded. Hence, the second term represents $(\prod_{j=k+1}^{n}L_j)$ sets of sliced tensor networks, each coded by 2-node code on its $k$ sliced 2-node indices.




For the case where the sliced indices all connect more than 2 nodes, partial coding for only one index with the least node connection might provide smaller $f$-resilient number compared to coding for all the sliced indices by Theorem 1. 

% In addition, although gain in $f$-resilient number is proportional to both number of node failures $f$ and sliced tensor networks $n$, gain from coding scheme of Theorem~\ref{thm:main} might be not good enough for certain distributed system and tensor networks. For instance, there could be a case where $f$ is not significantly large compared to the product term of $\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)}$. For such cases, we suggest corollary \ref{cor:partial1} and \ref{cor:partial2} each from theorem \ref{thm:main} and \ref{thm:2-node} respectively.

\begin{corollary}
(Partial Coding One Index) For the problem stated in \ref{sec:system}, if there are no 2-node indices among $n$ sliced indices, the achievable $f$-resilient number is bounded above by
\begin{equation}
\min \bigg(f+\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)},\hspace{5pt}(\prod_{j=2}^{n}L_j)(f+\sum_{k=1}^{L_1}m_1^{k-1})\bigg),
\end{equation}
where $m_1$ is the minimum of the $m_i (i=1,2,..,n)$
\end{corollary}



Note that the second term in $\min$ is the $f$-resilient number of coding one index with the least node connection and letting the other $(n-1)$ indices to slice without coding. Hence, there would be $\prod_{i=2}^{n} L_i$ sets of sliced tensor networks and each of them is coded for one index by Theorem 1.

For the case where some of the sliced indices are 2-node indices, partial coding for only 2-node indices might provide smaller $f$-resilient number compared to coding for all the sliced indices by Theorem 1. 

\begin{corollary}
(Partial Coding $k$ 2-node Indices) For the problem stated in \ref{sec:system}, if $m_i=2 (i=1,2,..,k)$ and $m_i>2(i=k+1,..,n$), the achievable $f$-resilient number is bounded above by
\begin{equation}
\min\bigg(f+\prod_{i=1}^{n}\frac{(m^{L_{i}}_{i}-1)}{(m_{i}-1)},\hspace{5pt}(\prod_{j=k+1}^{n}L_j)(f+\prod_{l=1}^{k}L_{l}-1)\bigg).
\end{equation}
\end{corollary}

We obtain the second term in $\min$ by encoding $k$ 2-node sliced indices and leaving the remaining $(n-k)$ indices uncoded. Hence, there are $(\prod_{j=k+1}^{n}L_j)$ sets of sliced tensor networks which each is coded for 2-node indices by Theorem 2.

==> system_problem.tex <==
\subsection{System model}\label{sec:system}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/systemmodel.pdf}
    \caption{\small{($\boldsymbol{a}$) System model for distributed parallel tensor network contraction without coding. Failure on any computational node will result as a failure of entire system ($\boldsymbol{b}$) System model for distributed coded parallel tensor network contraction. Even with some node failures, as long as the number of successful computational nodes is over recovery threshold, desired final outcome will always be retrieved.}}
    \label{fig:system}
    \vspace{-7pt}
\end{figure*}

Almost exactly same with the coded matrix multiplication. Replacing original sliced tensor networks by encoded sliced tensor networks, if recovery threshold number of nodes are successful, original final outcome can be retrieved at any case

\subsection{Problem Statement}\label{sec:problem}

In this paper, we provide algorithm-based fault tolerant coded computation strategies for parallel tensor network contraction scheme first proposed by Chen and Zhang\cite{chenzhang}, and explained in \ref{sec:para}. Using distributed computational system modeled in \ref{sec:system} and visualized in Fig. \ref{fig:system}, we are required to compute final outcome of an arbitrary tensor network. The tensor network is sliced by $n$ indices, which are each $m_{i}$-node, $L_{i}$ dimensional index ($i={1,2,\ldots,n}$). Hence, there are ($N=\prod_{i=1}^{n}L_{i}$) sliced tensor networks and we need all the individual contraction results from every one of them to sum up to acquire the final outcome of original network. For a system with $f$ node failures, if failures happen in an adversarial manner, all the sliced networks need naive replication by the number of $(f+1)$ to ensure at least one successful computational node exists for every one of them. Thus, recovery threshold for naive replication is as follows:
$$N(f+1),$$
where $N=\prod_{i=1}^{n}L_{i}$.

Hence, the main problem we solve in this paper is:
\begin{tcolorbox}{\begin{center}$\textit{{Problem Statement}}$\end{center}}

For a tensor network sliced by $n$ non-adjacent indices, each of  $m_{i}$-node and $L_{i}$ dimensional ($i={1,2,\ldots,n}$), achieve recovery threshold smaller than $N(f+1)$ using system model of \ref{sec:system} and distributed parallel algorithm of \ref{sec:para}\cite{chenzhang}, where $N=\prod_{i=1}^{n}L_{i}$. By the argument of \ref{sec:comp}\cite{markovshi}, encoded tensor networks must have the exact same topology as the sliced tensor networks.
\end{tcolorbox}

Reason why we formulate the problem for only non-adjacent sliced indices is to restrict structural freedom of an arbitrary tensor network. If we allow sliced indices to be adjacent to each other in an arbitary manner, problem will have infinite combinatorial freedom on its coding scheme. Justification on our restriction is from the recent work of step-dependent heuristics on searching indices to slice\cite{stepdependent}. In this work, indices are not selected altogether at the same step, but they are selected one by one interleaved by running contraction ordering heuristics. At each step of searching for an index to slice, an index that is approximated to reduce the computational complexity the most is chosen. Hence we assume that indices connected to tensors sliced in previous steps are likely to be less attractive, as the contraction cost of its contraction is already reduced from previous slicing. If one or more of the tensors connected to the index has lost its index from previous slicing steps, dimension of the intermediate tensor is reduced accordingly, hence that index has become cheaper to contract. However, we would like to emphasize that our assumptions can significantly fail for certain specific cases, and that both indices connecting fewer tensors than others and indices that are adjacent to each other can turn out to be close to optimal to slice for parallelization scheme. Hence, coding schemes for tensor networks allowing adjacent indices to be sliced are left for future works.

==> tncontraction.tex <==
\subsection{Tensor Network Concepts}

Tensor network has been developed to provide mathematical formalism for complex quantum many-body states\cite{quantummanybodyex1,quantummanybodyex2,quantummanybodyex3,quantummanybodyex4,quantummanybodyex5,quantummanybodyex6,quantummanybodyex7,quantummanybodyex8,quantummanybodyex9,quantummanybodyex10}, yet has also been proved to be a powerful framework for other applications such as machine learning\cite{mlexample1,mlexample2,mlexample3,mlexample4} and quantum circuit simulation.\cite{markovshi,boixo,qcsex1,qcsex2,bigbatch,adaptive,exa,indexslicing,jet,stepdependent,chenzhang}. Especially for quantum circuit simulation, ever since firstly proposed by the seminal work of Markov and Shi\cite{markovshi} then developed by Boixo\cite{boixo} and others\cite{adaptive}, tensor network formalism has significantly expanded the classical limit to simulate several quantum computing problems in past few years, such as QAOA algorithm\cite{qaoa} and random quantum circuit sampling\cite{randomcircuit}, which were originally regarded as NP-hard tasks for classical computers\cite{quantumsupremacy1,quantumsupremacy2}. Reasons why it is such a powerful and effective framework are well explained in numerous references cited above, and the topic itself is out of the scope of this work. Yet mathematically, tensor network is an extremely expressive framework for arbitrary linear algebraic operations and let us provide brief overview on its diagrammatic and mathematical representation.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/diagram.pdf}
    \caption{\small{Diagrammatic representation and corresponding array for ($\boldsymbol{a}$) one dimensional tensor $\boldsymbol{A}_{i}$ ($\boldsymbol{b}$) two dimensional tensor $\boldsymbol{B}_{i,j}$ ($\boldsymbol{c}$) three dimensional tensor $\boldsymbol{C}_{i,j,k}$}}
    \label{fig:diagram}
    \vspace{-7pt}
\end{figure}

As matrix multiplication can be considered as a generalization of inner product operation between one dimensional tensors for two dimensional tensors, or matrices, tensor network can be considered as a generalization of matrix multiplication for higher dimensional tensors. Tensor network consists of nodes and edges, where each node represents a tensor, and each edge connected to the node represents the index of the tensor. Diagrammatic representations of one dimensional tensor $\boldsymbol{A}_{i}$, two dimensional tensor $\boldsymbol{B}_{i,j}$, and three dimensional tensor $\boldsymbol{C}_{i,j,k}$ are shown in Fig \ref{fig:diagram}. In this paper, we will denote a tensor in bold text to differentiate from scalar. For the case of Fig. \ref{fig:diagram}$(c)$, let the index $i$ span as $\{1,2,3\}$ and if you fix the value of index $i$ as $1$, $\boldsymbol{C}_{1,j,k}$ is now a two dimensional tensor, the matrix at the top of the stack in Fig. 1($c$). It goes same for other indices $j$ and $k$, which fixing either of them by its value will \textit{slice} the tensor $\boldsymbol{C}_{i,j,k}$ to be a sheet of two dimensional tensor. We will use the term \textit{slice} as fixing the value of the index for the rest of the paper. Tensor can be sliced multiple times as many as indices it has, for example if $\boldsymbol{C}_{i,j,k}$ is sliced by index $i$ and $j$, resulting sliced tensor is one dimensional vector with remaining index of $k$.

If an edge is shared by two or more different nodes in a tensor network diagram, that means the corresponding index is shared by its connected tensors in the network. There are two types of edges in the formalism, open edge and closed edge. Each closed edge is to be contracted individually by the product sum operation analogous to inner product by the index it represents. This operation is referred as \textit{contraction}, which is done sequentially by all closed edges one by one until none of it remains in the network. At the end, a single node will remain. The resulting node is the final outcome of the tensor network, so a tensor network ends up as a single tensor eventually. All open edges remain to be the edges of the final node, hence they represent indices of the final tensor.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/contraction.pdf}
    \caption{\small{Diagrammatic representation of tensor network contraction for ($\boldsymbol{a}$) $\sum_{j}\boldsymbol{A}_{i,j}\boldsymbol{B}_{j,k}$   ($\boldsymbol{b}$) $\sum_{k,j,l}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l}\boldsymbol{C}_{c,l,j}$  
 ($\boldsymbol{c}$) $\sum_{j}\boldsymbol{A}_{j,a}\boldsymbol{B}_{b,j}\boldsymbol{C}_{j,c}$}}
    \label{fig:contraction}
    \vspace{-7pt}
\end{figure}

For instance, let us demonstrate a simple tensor network representing matrix multiplication. Fig. 2($a$) shows a tensor network with two nodes each representing tensor $\boldsymbol{A}_{i,j}$ and $\boldsymbol{B}_{j,k}$ respectively, connected by one closed edge representing their shared index $j$. Indices $i$ and $k$ are open edges each connected to its tensors. Then, contraction by the closed edge representing $j$ results as a single node with two open edges remaining, representing the final tensor $\boldsymbol{C}_{i,k}$ with indices $i$ and $k$. Equation of the contraction is as follows:
$$\sum_{j}\boldsymbol{A}_{i,j}\boldsymbol{B}_{j,k}=\boldsymbol{C}_{i,k}.$$
This is matrix multiplication as we know, represented by tensor network formalism. Note that the closed edge of index $j$ disappears in the network after its own contraction, hence the term \textit{contraction}. Let us use \textit{node} and \textit{tensor} interchangeably, and \textit{edge} and \textit{index} as well for convenience and readability. We will clarify when the term \texit{node} is used to refer computational node to not leave any confusion.

Another simple tensor network is shown as a diagram in Fig. 2($b$) Now it has three tensors $\boldsymbol{A}_{a,j,k}$, $\boldsymbol{B}_{b,k,l}$, and $\boldsymbol{C}_{c,l,j}$, with three closed indices $j$, $k$, $l$, and three open indices $a$, $b$, $c$. There are three contraction to be done for this network, as there are three closed edges. Let us do the contraction by the order of $(k,l,j)$. First contraction by index $k$ goes as follows:
$$\sum_{k}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l}\boldsymbol{C}_{c,l,j}=(\sum_{k}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l})\boldsymbol{C}_{c,l,j},$$
where $(\sum_{k}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l})$ can be represented as a single tensor with four indices $(a,j,b,l)$.
$$(\sum_{k}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l})=\boldsymbol{T}^{(1)}_{a,j,b,l}$$
This tensor $\boldsymbol{T}^{(1)}_{a,j,b,l}$ is called an intermediate tensor, as it is produced by an intermediate step of sequential contractions in progress. After this first contraction by $k$, tensor network has two tensors $\boldsymbol{T}^{(1)}_{a,j,b,l}$ and $\boldsymbol{C}_{c,l,j}$, connected by two closed indices $j$ and $l$. Second contraction by $l$ is as follows, producing another intermediate tensor:
$$\sum_{l}\boldsymbol{T}^{(1)}_{a,j,b,l}\boldsymbol{C}_{c,l,j}=\boldsymbol{T}^{(2)}_{a,j,b,c}.$$
After second contraction, only one tensor is left in the network, yet one last closed index is left as well. This index can be represented as a closed loop connected to only one tensor. Last contraction by the index $j$ is as follows:
$$\sum_{j}\boldsymbol{T}^{(2)}_{a,j,b}=\boldsymbol{T}^{(\text{final})}_{a,b,c}.$$
Including all three contractions, the tensor network can be mathematically represented as follows:
$$\sum_{k,j,l}\boldsymbol{A}_{a,j,k}\boldsymbol{B}_{b,k,l}\boldsymbol{C}_{c,l,j}=\boldsymbol{T}^{(\text{final})}_{a,b,c}.$$
Note that it ends up as a single tensor with all the open indices from the original tensor network. Also, contraction order does not change the outcome of the network. Whether sequential contraction is done by the sequence of $(k,l,j)$, $(k,j,l)$ or by other order possible, does not change the final tensor $\boldsymbol{T}^{(\text{final})}_{a,b,c}$.

We had only provided examples with indices connecting two tensors, but the expressive nature of tensor network also allows index shared by more than two tensors. Fig. 2($c$) shows a tensor network with three tensors all sharing an index $j$. Each of the tensors has one open indices of $a$, $b$, and $c$, so the final tensor will be a three dimensional tensor with indices $(a,b,c)$. Contraction by index $j$ is as follows:
$$\sum_{j}\boldsymbol{A}_{j,a}\boldsymbol{B}_{b,j}\boldsymbol{C}_{j,c}=\boldsymbol{T}^{\text{final}}_{a,b,c}.$$

Open indices remaining after each contraction either on an intermediate tensor or on the final tensor need to be fixed by every combination possible to fill up the resulting tensor. For instance, from the previous example of Fig. 2($c$), final tensor $\boldsymbol{T}^{\text{final}}_{a,b,c}$ is a three dimensional tensor with number of elements as many as the possible combination of $(a,b,c)$. And the product sum must be done on each elements of the final tensor. For example, to fill up an element corresponding to $(a=1,b=1,c=1)$ of the final tensor, open indices $(a,b,c)$ must be fixed accordingly in the original tensor network before the contraction.
$$\boldsymbol{T}_{1,1,1}=\sum_{j}\boldsymbol{A}_{j,1}\cdot\boldsymbol{B}_{1,j}\cdot\boldsymbol{C}_{j,1}$$
This is same for any intermediate step of sequential contractions. As you can see, number of open indices of the resulting tensor from a contraction dictates the computational complexity of the contraction. Let us say the dimension of the indices of the network in Fig. 2($c$) is $L$. Or, we can say the maximum dimension of the indices is $L$. Then the computational complexity of contraction by $j$ is exponential to $L$, by the number of open indices and plus one, as there are terms in the product sum as many as the dimension of contracted index $j$. Hence, the computational complexity is $O(L^{3+1})=O(L^4)$ for this case.

In a nutshell, tensor network is an extremely expressive formalism that represents arbitrary product sum operations for arbitrary tensors by arbitrary connections of indices between them. More detailed tutorials and explanations on tensor network concepts and its applications can be found in following references\cite{tnguide,nutshell,quantummanybodyex4}. By itself, it is memory efficient to represent a complex quantum many-body system often with numerous entanglements. A very simple yet intuitive example for its memory efficiency can be the representation of a 4-qubit state by a tensor product of two 2-qubit states. If a 4-qubit system consists of two 2-qubit states unentangled to each other, it can be represented as a tensor product between them. Each 2-qubit states may or may not be an entangled state of single qubits consisting them. If the 4-qubit state is represented as a state vector, you need $16$ elements in that vector as the state is $2^4$ dimensional. However, if represented as a tensor product of two 2-qubit states, which each is a $2^2$ dimensional, you only need $8$ elements to represent the state.

Another crucial property of tensor network is that its contraction can be done by embarrassingly parallel algorithm, first demonstrated in the work of Chen and Zhang\cite{chenzhang}. It can fully exploit the workforce of a large scale distributed system, and its parallelization has shown numerous breakthroughs in the field of quantum circuit simulation\cite{indexslicing,stepdependent,jet}. This property is the central focus of our work, to provide fault tolerant coding algorithm for distributed parallel tensor network contraction.



\subsection{Computational complexity of contraction}\label{sec:complexity}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/sampletn.pdf}
    \caption{\small{Diagrammatic representation of sample tensor network $\sum_{i,j,k,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,k}\boldsymbol{C}_{j,l}\boldsymbol{D}_{k,l}\boldsymbol{E}_{k,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$}}
    \label{fig:sampletn}
    \vspace{-7pt}
\end{figure}

Before explaining parallel tensor network contraction, we briefly explain how computational complexity can be evaluated for a tensor network. Fig. 3 shows a sample network we will use to explain the arguments. Mathematical representation of the network would be as follows:
$$\sum_{i,j,k,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,k}\boldsymbol{C}_{j,l}\boldsymbol{D}_{k,l}\boldsymbol{E}_{k,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g} = \boldsymbol{T}^{\text{final}}_{f,g}$$

As explained in the previous section, this network has to go through sequential contractions by six closed edges. Although the final tensor resulting at the end will be the same regardless of the order of contractions, a set of intermediate tensors produced by each ordering is different. For instance, if the closed index $i$ is contracted first, tensor $\boldsymbol{A}_{i}$ and $\boldsymbol{B}_{i,j,k}$ is contracted to an intermediate tensor $\boldsymbol{T}^{1}_{j,k}$. This contraction has the computational complexity of $O(L^3)$. However, if the first contraction is done by index $k$, tensors $\boldsymbol{B}_{i,j,k}$, $\boldsymbol{D}_{k,l}$, and $\boldsymbol{E}_{k,m}$ will be contracted to produce an intermediate tensor $\boldsymbol{T}^{1}_{i,j,l,m}$. Then, the computational complexity of this contraction is $O(L^5)$, two order of magnitude larger than the previous case.

It is easy to see that if the contraction order is wisely chosen, all the contractions have a smaller computational complexity than $O(L^5)$. For instance, if the contraction is done by the order of $(i,j,k,l,m,n)$, maximum number of open indices for the intermediate tensors resulting from each contraction is $3$. Hence, the computational complexity of contracting the entire tensor network is polynomial to $O(L^4)$. However, for contraction ordering with index $k$ at the beginning, the sample network has the computational complexity polynomial to $O(L^5)$. This means there exists an optimal order of contraction for a given tensor network. However, finding the optimal contraction order for an arbitary tensor network is a NP-complete problem\cite{markovshi}.

Although there is no general algorithm to evaluate the exact minimum computational complexity of a given tensor network, by far many effective heuristic algorithms have been developed to approximate the minimum complexity and find contraction order close to optimal\cite{hyperoptimized,simpleheuristic,adaptive,arbitrarycontract}. Seminal work of Markov and Shi\cite{markovshi} proved that the minimum computational complexity of a given tensor network is exponential to the \textit{treewidth} of the network, which is a graph theoretic property of the line graph representation of the network. Calculating treewidth of a tensor network is another NP-hard combinatorial problem, but the work of Markov and Shi\cite{markovshi} provides us a very important insight that the topology of a tensor network decides its minimum computational complexity. In other words, this means tensor networks with exactly same topology have similar computational cost when independently computed by identical computational nodes.


\subsection{Parallel tensor network contraction}\label{sec:parallel}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/parallel.pdf}
    \caption{\small{Parallelization scheme by index $k$ for sample tensor network of Fig. \ref{fig:sampletn}}}
    \label{fig:parallel}
    \vspace{-7pt}
\end{figure}


First demonstrated by the work of Chen and Zhang\cite{chenzhang}, tensor network contraction can be distributed to multiple independent computational nodes by embarrassingly parallel algorithm. For instance, sample tensor network of Fig. 3 can be \textit{sliced} by the index $k$ and partitioned into $L$ sliced tensor networks. This is in fact a simple expansion of the mathematical representation of the network by the index $k$. Let us say index $k$ span as $\{1,2,...,L\}$. Then, the equation for the network can be expanded by index $k$ as follows:
$$\sum_{i,j,k,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,k}\boldsymbol{C}_{j,l}\boldsymbol{D}_{k,l}\boldsymbol{E}_{k,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$$
$$=\sum_{i,j,l,m,n}(\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,1}\boldsymbol{C}_{j,l}\boldsymbol{D}_{1,l}\boldsymbol{E}_{1,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g})$$
$$+\sum_{i,j,l,m,n}(\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,2}\boldsymbol{C}_{j,l}\boldsymbol{D}_{2,l}\boldsymbol{E}_{2,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g})$$
$$\vdots$$
$$+\sum_{i,j,l,m,n}(\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,L}\boldsymbol{C}_{j,l}\boldsymbol{D}_{L,l}\boldsymbol{E}_{L,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g})$$
The equation is now represented as $L$ different terms where the tensors ($\boldsymbol{B}_{i,jk,}$, $\boldsymbol{D}_{k,l}$, $\boldsymbol{E}_{k,m}$) are replaced by each fixed values of index $k$. 

Each term can represent an independent tensor network by itself, which can be contracted independently. If each sliced tensor networks is distributed to an individual computational nodes, its contraction does not require any communication with other nodes thus the distributed computation is embarrassingly parallel. For computational node $i$, we denote the resulting tensor from the sliced tensor network as $\{\boldsymbol{\sigma}_{i}\}$ as follows:
$$\boldsymbol{\sigma}_{1} = \sum_{i,j,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,1}\boldsymbol{C}_{j,l}\boldsymbol{D}_{1,l}\boldsymbol{E}_{1,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$$
$$\boldsymbol{\sigma}_{2} = \sum_{i,j,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,2}\boldsymbol{C}_{j,l}\boldsymbol{D}_{2,l}\boldsymbol{E}_{2,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$$
$$\vdots$$
$$\boldsymbol{\sigma}_{L} = \sum_{i,j,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,L}\boldsymbol{C}_{j,l}\boldsymbol{D}_{L,l}\boldsymbol{E}_{L,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$$
Final outcome of the original tensor network, $\boldsymbol{T}^{\text{final}}_{f,g}$ from the previous subsection, can be denoted as $\boldsymbol{\sigma}_{\text{final}}$ and it is a summation of the partial results coming from the distributed computational nodes $(\boldsymbol{\sigma}_{1},\boldsymbol{\sigma}_{2},...,\boldsymbol{\sigma}_{L})$ as follows:
$$\boldsymbol{\sigma}_{\text{final}}=\boldsymbol{\sigma}_{1}+\boldsymbol{\sigma}_{2}+\ldots+\boldsymbol{\sigma}_{L}$$
In diagrammatic representation, sliced tensor networks replace the nodes representing the tensors ($\boldsymbol{B}_{i,j,k}$, $\boldsymbol{D}_{k,l}$, $\boldsymbol{E}_{k,m}$) with their sliced subtensors and erase the sliced index $k$. For instance, diagram for sliced tensor network $\boldsymbol{\sigma}_{1}$ replaces nodes ($\boldsymbol{B}_{i,j,k}$, $\boldsymbol{D}_{k,l}$, $\boldsymbol{E}_{k,m}$) in the original tensor network by ($\boldsymbol{B}_{i,j,1}$, $\boldsymbol{D}_{1,l}$, $\boldsymbol{E}_{1,m}$), and erase the edge $k$. As a result, all sliced tensor networks share exactly same topology with each other, hence the computational complexity is similar between them. Thus this parallelization algorithm enables to distribute original task into sliced subtasks with similar computational cost.

As much as efficient it is, this parallelization scheme has achieved great breakthroughs in the field of quantum circuit simulation\cite{indexslicing,stepdependent,jet}. However, in this work, we would like to focus on the extreme vulnerability of this algorithm for computational node failures. As the final outcome of the algorithm requires to retrieve every partial results from mutually independent computational nodes, if any of the worker nodes assigned with each sliced tensor network fail, our desired final outcome cannot be acquired. Straggler nodes with latency, error, and other undesirable malfunctioning degrade the efficiency of this embarrassingly parallel algorithm without any resilience. Considering the algorithm is mainly used for tasks that are at the verge of the classical limit, concurrent and prospective implementations of it are mostly aimed for exa-scale super clusters where multiple node failures are very likely to happen\cite{exa}. To our knowledge, we have not yet found any works concerning this problem. In this paper, we propose first ever attempt, as we know of, to make parallel tensor network contraction fault tolerant by coded computation strategies analogous to coded matrix multiplication.

\subsection{Notation}
Before explaining our coding strategies, let us define notations for equations we will use to refer tensor networks. What we are attempting to encode in this work are tensor networks sliced by one or more indices, all of them sharing common nodes and edges except for the nodes representing the sliced tensors. To keep equations straightforward and easy to read, we would like to simplify notations on the common nodes and edges between sliced tensor networks as much as possible, as they need to be written repeatedly without any significance. Hence, we omit all the irrelevant indices other than the sliced indices and denote them as $`-'$ in follows equations. Also, we represent all the shared tensors by a single tensor $\boldsymbol{T}_{-}$, as they are another partial tensor network of their own which can be contracted to be a single tensor. In addition, partial result from the contraction of each sliced networks will be denoted as $\boldsymbol{\sigma}$ with lower indent of the value of the sliced index.

For instance, equation for the sliced tensor network $\boldsymbol{\sigma}_{x}$ in the previous subsection,
$$\boldsymbol{\sigma}_{x} = \sum_{i,j,l,m,n}\boldsymbol{A}_{i}\boldsymbol{B}_{i,j,x}\boldsymbol{C}_{j,l}\boldsymbol{D}_{x,l}\boldsymbol{E}_{x,m}\boldsymbol{F}_{l,n,f}\textbf{G}_{m,n,g}$$
can be denoted as follows:
$$\boldsymbol{\sigma}_{1} = \sum_{-}(\boldsymbol{B}_{1,-}\boldsymbol{D}_{1,-}\boldsymbol{E}_{1,-})\boldsymbol{T}_{-}$$
$$\boldsymbol{\sigma}_{2} = \sum_{-}(\boldsymbol{B}_{2,-}\boldsymbol{D}_{2,-}\boldsymbol{E}_{2,-})\boldsymbol{T}_{-}$$
$$\vdots$$
$$\boldsymbol{\sigma}_{L} = \sum_{-}(\boldsymbol{B}_{L,-}\boldsymbol{D}_{L,-}\boldsymbol{E}_{L,-})\boldsymbol{T}_{-}$$
where the final outcome can be denoted as $\boldsymbol{\sigma}_{\text{final}}$:
$$\boldsymbol{\sigma}_{\text{final}} = \boldsymbol{\sigma}_{1}+\boldsymbol{\sigma}_{2}+\ldots+\boldsymbol{\sigma}_{L}.$$

Note that our notation does not mean that we intend to contract non-sliced indices. Our goal in this work is to encode each of the sliced tensor networks and achieve algorithm-based fault tolerant distributed computation of parallel tensor network contraction by our coded computation strategies.

In addition, for convenience and readability, let us refer to an index shared by $m$ different tensors as an \textit{m-node index}. In diagrammatic representation, the edge representing the index is connected to $m$ nodes, hence the term. Furthermore, we will define the indices of a tensor to be \textit{adjacent} to each other, as in diagrammatic representation edges they represent are connected to the same node. Hence \textit{non-adjacent} indices are each of different tensors.
